RE-SORT: Removing Spurious Correlation in Multilevel Interaction for CTR Prediction

Click-through rate (CTR) prediction is a critical task in recommendation systems, serving as the ultimate filtering step to sort items for a user. Most recent cutting-edge methods primarily focus on investigating complex implicit and explicit feature interactions; however, these methods neglect the spurious correlation issue caused by confounding factors, thereby diminishing the model's generalization ability. We propose a CTR prediction framework that REmoves Spurious cORrelations in mulTilevel feature interactions, termed RE-SORT, which has two key components. I. A multilevel stacked recurrent (MSR) structure enables the model to efficiently capture diverse nonlinear interactions from feature spaces at different levels. II. A spurious correlation elimination (SCE) module further leverages Laplacian kernel mapping and sample reweighting methods to eliminate the spurious correlations concealed within the multilevel features, allowing the model to focus on the true causal features. Extensive experiments conducted on four challenging CTR datasets and our production dataset demonstrate that the proposed method achieves state-of-the-art performance in both accuracy and speed. The utilized codes, models and dataset will be released at https://github.com/RE-SORT.

==> table/abtest.tex <==
\begin{table}[hb]
 \small
 \centering
  \begin{tabular}{c|c|c|c|c|c|c|c|c}
  \toprule
 \makebox [0.083\textwidth][c]{}  &  \makebox[0.083\textwidth][c]{Day1}  & \makebox[0.083\textwidth][c]{ Day2}      & \makebox[0.083\textwidth][c]{ Day3} & \makebox[0.083\textwidth][c]{ Day4}  & \makebox[0.083\textwidth][c]{ Day5}  & \makebox[0.083\textwidth][c]{ Day6}  & \makebox[0.083\textwidth][c]{ Day7} & \makebox[0.083\textwidth][c]{ Average}\\
\midrule
    $\triangle$ CTR    & 1.43\%    & 1.56\%  & 1.79\%  & 1.82\% & 1.78\% & 1.58\% & 1.37\% & 1.62\% \\
\bottomrule
  \end{tabular}
   \caption{Results of a seven-day online A/B test.}
 \label{abtest_7}
\end{table}

==> table/bias.tex <==
























% \begin{table*}[t]

%  \centering
%  \resizebox{\textwidth}{!}{
%  \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
%   \toprule
%   \multirow{2} * {\makebox[0.005\textwidth][c]{Model}} & 
% \multicolumn{2}{c|}{\makebox[0.1\textwidth][c]{$\rho=-3$}} &
% \multicolumn{2}{c|}{\makebox[0.1\textwidth][c]{$\rho=-2.5$}} &
% \multicolumn{2}{c|}{\makebox[0.1\textwidth][c]{$\rho=-1.5$}} &
% \multicolumn{2}{c|}{\makebox[0.1\textwidth][c]{$\rho=1.5$}} &
% \multicolumn{2}{c|}{\makebox[0.1\textwidth][c]{$\rho=2.5$ \textsuperscript{$\dagger$}}} &
% \multicolumn{2}{c}{\makebox[0.1\textwidth][c]{$\rho=3$}}\\
%   & AUC $\uparrow$    & Logloss $\downarrow$  & AUC $\uparrow$   & Logloss $\downarrow$  & AUC $\uparrow$    & Logloss $\downarrow$ & AUC $\uparrow$    & Logloss $\downarrow$  & AUC $\uparrow$    & Logloss $\downarrow$  & AUC $\uparrow$    & Logloss $\downarrow$\\
% \midrule

%     Baseline            & 0.7008   & 0.48    & 0.7326  & 0.47   & 0.7491   & 0.52   & 0.7831  & 0.48   & 0.8033  & 0.4064   & 0.7818  & 0.4147  \\
%     GDCN                & 0.7082   & 0.47    & 0.7436  & 0.46   & 0.7541   & 0.48   & 0.7873  & 0.45   & 0.8037  & 0.4055   & 0.7865  & 0.4135  \\
%     CFM                 & 0.7117   & 0.48    & 0.7498  & 0.47   & 0.7623   & 0.51   & 0.7855  & 0.47   & 0.8032  & 0.4070   & 0.7849  & 0.4139  \\
%     LightDIL            & 0.7248   & 0.48    & 0.7542  & 0.47   & 0.7641   & 0.51   & 0.7860  & 0.47   & 0.8035  & 0.4066   & 0.7866  & 0.4135  \\
%     Baseline + SCE      & 0.7403   & 0.44    & 0.7637  & 0.43   & 0.7691   & 0.45   & 0.7903  & 0.42   & 0.8053  & 0.4035   & 0.7882  & 0.4130  \\
% \midrule
%    RE-SORT
%   & \textbf{0.7450  }\textsuperscript{$\star$$\star$}
%   & \textbf{        }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.7694  }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.4     }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.7759  }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.43    }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.7943  }\textsuperscript{$\star$$\star$}
%   & \textbf{0.4190  }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.8058  }\textsuperscript{$\star$$\star$}
%   & \textbf{0.40    }\textsuperscript{$\star$$\star$} 
%   & \textbf{0.7931  }\textsuperscript{$\star$$\star$}
%   & \textbf{0.40    }\textsuperscript{$\star$$\star$}  
%     \\ 
%     Rel. Imp & 0.0490  & -0.0483  &0.0428   &-0.0430  &0.0525  & -0.0530  & 0.0390 & -0.0394 & 0.0021 & -0.0028  &0.0483  & -0.0479 \\
% \bottomrule
%  \end{tabular} 
%   }
%  \caption{ Comparative analysis in the IID and OOD settings. We utilize the UGC data with $\rho=2.5$ as the training data. \textsuperscript{$\dagger$}: the testing data with $\rho=2.5$ can be regarded as the in distribution data. As the parameter $\rho$ increases, the difference in distribution between the testing and training datasets also increases. ``Rel. Imp'' denotes the relative improvements compared with the LightDIL.
%  }
%  \label{bias}

 
% \end{table*}


==> table/different_block.tex <==
% \begin{table*}[ht]
% \small
%  \centering
%  \begin{tabular}{c|cc|cc|cc|cc|cc}
%   \toprule
%   \multirow{2} * {\makebox[0.09\textwidth][c]{Model}} & 
%   \multicolumn{2}{c|}{\makebox[0.12\textwidth][c]{Block number = 1}} & 
%   \multicolumn{2}{c|}{\makebox[0.12\textwidth][c]{Block number = 2}} & 
%   \multicolumn{2}{c|}{\makebox[0.12\textwidth][c]{Block number = 3}} &
%   \multicolumn{2}{c|}{\makebox[0.12\textwidth][c]{Block number = 4}} & 
%   \multicolumn{2}{c}{\makebox[0.12\textwidth][c]{Param.}} \\
%    & Criteo & UGC & Criteo & UGC & Criteo & UGC & Criteo & UGC & Criteo & UGC\\
% \midrule
%    MLP block       & 0.8110  & 0.8004 & 0.8117  & 0.8014 & 0.8115 & 0.8012 & 0.8112 &  0.8007 & 4.8M &\\
%    SA block & 0.8115 & 0.8011 & 0.8125 & 0.8019 & 0.8123  & 0.8017& 0.8119 & 0.8015            & 5.3M &\\
% \midrule
%    RE block  & \textbf{0.8128}\textsuperscript{$\star$$\star$} & \textbf{0.8018}\textsuperscript{$\star$$\star$} & \textbf{0.8133}\textsuperscript{$\star$$\star$} & \textbf{0.8021}\textsuperscript{$\star$$\star$} & \textbf{0.8136}\textsuperscript{$\star$$\star$} & \textbf{0.8028}\textsuperscript{$\star$$\star$} & \textbf{0.8132}\textsuperscript{$\star$$\star$} & 
%    \textbf{0.8024} \textsuperscript{$\star$$\star$} & 3.5M&\\
% \bottomrule
%  \end{tabular} 
%  \caption{ Performance (AUC) comparison among our proposed stacked recurrent (RE) block, the stacked MLP block, and the stacked self-attention (SA) block within a single stream. The last column shows the parameters (``Param.'') of each block. The implementations of different types of blocks can be found in our open-source code.
%  }
%  \label{different_block}
% \end{table*}



















\begin{table*}[ht]
\small
 \centering
 \begin{tabular}{c|cc|cc|cc|cc}
  \toprule
  \multirow{2} * {\makebox[0.18\textwidth][c]{Model}} & 
  \multicolumn{2}{c|}{\makebox[0.17\textwidth][c]{Block number = 1}} & 
  \multicolumn{2}{c|}{\makebox[0.17\textwidth][c]{Block number = 2}} & 
  \multicolumn{2}{c|}{\makebox[0.17\textwidth][c]{Block number = 3}} &
  \multicolumn{2}{c}{\makebox[0.17\textwidth][c]{Block number = 4}} \\
   & Criteo & UGC & Criteo & UGC & Criteo & UGC & Criteo & UGC \\
\midrule
   MLP block       & 0.8110  & 0.8004 & 0.8117  & 0.8014 & 0.8115 & 0.8012 & 0.8112 &  0.8007 \\
   SA block & 0.8115 & 0.8011 & 0.8125 & 0.8019 & 0.8123  & 0.8017& 0.8119 & 0.8015\\
\midrule
   RE block  & \textbf{0.8128}\textsuperscript{$\star$$\star$} & \textbf{0.8018}\textsuperscript{$\star$$\star$} & \textbf{0.8133}\textsuperscript{$\star$$\star$} & \textbf{0.8021}\textsuperscript{$\star$$\star$} & \textbf{0.8136}\textsuperscript{$\star$$\star$} & \textbf{0.8028}\textsuperscript{$\star$$\star$} & \textbf{0.8132}\textsuperscript{$\star$$\star$} & 
   \textbf{0.8024} \textsuperscript{$\star$$\star$}\\
\bottomrule
 \end{tabular} 
 \caption{ Performance (AUC) comparison among our proposed stacked recurrent (RE) block, the stacked MLP block, and the stacked self-attention (SA) block within a single stream. The implementations of different types of blocks can be found in our open-source code.
 }
 \label{different_block}
\end{table*}

